Efficient Computation of Trip-based Group Nearest Neighbor Queries (Full Version)

In recent years, organizing group meetups for entertainment or other necessities has gained significant importance, especially given the busy nature of daily schedules. People often combine multiple activities, such as dropping kids off at school, commuting to work, and grocery shopping, while seeking opportunities to meet others. To address this need, we propose a novel query type, the Trip-based Group Nearest Neighbor (T-GNN) query, which identifies the optimal meetup Point of Interest (POI) that aligns with users' existing trips. An individual trip consists of a sequence of locations, allowing users the flexibility to detour to the meetup POI at any location within the sequence, known as a detour location. Given a set of trips for the users, the query identifies the optimal meetup POI (e.g., restaurants or movie theaters) and detour locations from each user's trip that minimize the total trip overhead distance. The trip overhead distance refers to the additional distance a user must travel to visit the meetup POI before returning to the next location in their trip. The sum of these overhead distances for all users constitutes the total trip overhead distance. The computation time for processing T-GNN queries increases with the number of POIs. To address this, we introduce three techniques to prune the POIs that cannot contribute to the optimal solution, and thus refine the search space. We also develop an efficient approach for processing T-GNN queries in real-time. Extensive experiments validate the performance of the proposed algorithm.

==> sections/8_Biography.tex <==
\section{}{\label{biography}}
\begin{IEEEbiographynophoto}{Shahiduz Zaman}
received her B.Sc. and M.Sc. degree in Computer Science and Engineering from Bangladesh University of Engineering and Technology. She is currently a PHD student in the same institution. Her major research interest is spatial data, data engineering, deep learning on network data.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Tanzima Hashem}

\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Sukarna Barua}

\end{IEEEbiographynophoto}

==> sections/algos/baseline.tex <==

\KwIn{POI $p$ location list $L_i$ user $u_i$}
\KwOut{minimum overhead distance $min_i$ for the users and user will travel to the POI $p$ from location $dp_i$}

		 
	      $min_i \gets \infty$ \;
		%$\{min, dp\} \gets  find\_closest\_adjacent\_pair\_with\_dist(p, L_i)$\;               
	      \For{$j \gets 1$ to  $sizeof(L_i)$}{

			$OD \gets d(l_i^j, p) + d(l_i^{j+1}, p) - d(l_i^j, l_i^{j+1})$\;
			\If{ $min_i > OD$}{
				$min_i \gets OD$ \; 	
				$dp_i \gets l_i^j$\;
			}

		}
		


		%%%%%%%%%%%%%%%%%%%%%%%%
		%$tl_i \gets \emptyset$\;
		%\For{$i \gets 1$ to $n$}{     
		%	 $min_i \gets \infty$ \;               
		 %     \For{$j \gets 1$ to  $sizeof(L_i)$}{
		%		$OD \gets Dist_{min}(l_i^j, p) + Dist_{min}(l_i^{j+1}, p) - Dist_{min}(l_i^j, l_i^{j+1})$\;
		%		\If{ $j = 1$ or $min_i > OD$}{
		%			$min_i \gets OD$ \; 
		%			$tl_i \gets j$\;
		%		}
		%	}
		%}
		%%%%%%%%%%%%%%%%%%%%%%%%


\Return \{$min_i, dp_i$\}\;



==> sections/algos/calculate_min.tex <==

% \KwIn{Meetup POI $p$ and trip locations $L_i$ for user $u_i$}
% \KwOut{Minimum overhead distance $TO_i$ and detour location $l^d_i$ for user $u_i$}
\KwIn{$\{p, L_i\}$ }
\KwOut{$\{TO_i, l^d_i\}$}

	      $TO_i \gets \infty$ \;
		%$\{min, dp\} \gets  find\_closest\_adjacent\_pair\_with\_dist(p, L_i)$\;               
	      \For{$j \gets 1$ to  $sizeof(L_i)-1$}{
			$OD \gets d(l_i^j, p) + d(l_i^{j+1}, p) - d(l_i^j, l_i^{j+1})$\;
			\If{ $OD < TO_i$}{
				$TO_i \gets OD$ \; 	
				$l^d_i \gets l_i^j$\;
			}
		}
		


		%%%%%%%%%%%%%%%%%%%%%%%%
		%$tl_i \gets \emptyset$\;
		%\For{$i \gets 1$ to $n$}{     
		%	 $min_i \gets \infty$ \;               
		 %     \For{$j \gets 1$ to  $sizeof(L_i)$}{
		%		$OD \gets Dist_{min}(l_i^j, p) + Dist_{min}(l_i^{j+1}, p) - Dist_{min}(l_i^j, l_i^{j+1})$\;
		%		\If{ $j = 1$ or $min_i > OD$}{
		%			$min_i \gets OD$ \; 
		%			$tl_i \gets j$\;
		%		}
		%	}
		%}
		%%%%%%%%%%%%%%%%%%%%%%%%


\Return \{$TO_i, l^d_i$\}\;



==> sections/algos/compute_static_distance.tex <==
\KwIn{$\{\mathcal{L}, c\}$
%The set of users' trip locations $\mathcal{L}=\{L_1, L_2, ...,L_n\}$ and the center of each user
}
\KwOut{$\{T[1..n], mdist[1..n], cdist[1..n]\}$
% Return $T[1..n]$: trip distance of each user without visiting any POI, $mdist[1..n]$: maximum distance between two adjacent locations for each user, and $cdist[1..n]$: maximum euclidean distance between a trip location and the trip centroid for each user
}
    \For{$i\leftarrow 1..n$}{ 
        $mdist[i] \leftarrow 0$\;
        $cdist[i] \leftarrow 0$\;
        $T[i] \leftarrow 0$\;
        \For{$j\leftarrow 1..m_i$}{
                \If{$j < m_i$}{
                    $tempDist\leftarrow d(l_i^j, l_i^{j+1})$\;
                    $T[i] \leftarrow T[i] + tempDist$\;
                    \If{$mdist[i] < tempDist$}{
                        $mdist[i] \leftarrow tempDist$\;
                    }
                }
                \If{$cdist[i] < d_E(l_i^j, c_i)$ }{
                    $cdist[i] \leftarrow d_E(l_i^j, c_i)$\;
                }
        }
    }
\Return \{$T[1..n], mdist[1..n], cdist[1..n]$\}\;



==> sections/algos/is_include.tex <==

\KwIn{$\{c_K, r_K, S_1, S_2, S_3\}$}
\KwOut{$\{true/false\}$}
% \KwOut{It returns $true$ if circular region centered at $c_K$ with radius $r_K$ covers at least one of search region}

$C_K\leftarrow Circle(c_K, r_K)$\;
\If{$S_1$ is inside $C_K$}{
	\Return $true$\;
}
\If{$S_2$ is inside $C_K$}{
	\Return $true$\;
}
\If{$S_3$ is inside $C_K$}{
	\Return $true$\;
}
\Return $false$\;



==> sections/algos/is_prune.tex <==

\KwIn{$\{p, S_1, S_2, S_3\}$}
\KwOut{$\{true/false\}$}
% \KwOut{It returns $true$ if POI $p$ can be pruned else it returns $false$}

\If{$p$ is outside $S_1$}{
		\Return $true$\;
	}
	\If{$p$ is outside $S_2$}{
		\Return $true$\;
	}
	\If{$p$ is outside $S_3$}{
		\Return $true$\;
	}
\Return $false$\;



==> sections/algos/t_gnn.tex <==

% \KwIn{$\{\mathcal{L}, root\}$, where $\mathcal\{\mathcal{L}\}=\{L_1,L_2,\dots,L_n\}$ is the set of users' trip locations and $root$ is the root node of the R*-tree}
% \KwOut{$R=\{p, L^d\}$ where $p$ is the meetup POI and $L^d=\{l^d_1, l^d_2, \dots, l^d_n\}$ is the set of detour locations}
\begin{algorithmic}[1]
\KwIn{$\{\mathcal{L}, root\}$}
\KwOut{$R=\{p, L^d\}$}
$TO_{opt} \gets \infty$, $L^d \gets \phi$\;
\For{$i\leftarrow 1..n$}{                    
        $c_i\leftarrow \frac{1}{m_i}\sum_{j=1}^{m_i}{l_i^j}$\;
        $S_1[i].center = c_i, S_2[i].center = c_i, S_3[i].center = c_i$\;
        $S_1[i].radius = \infty, S_2[i].radius = \infty, S_3[i].radius = \infty$\;
}
$c_K\leftarrow \frac{1}{n}\sum_{j=1}^{n}{c_j}$,  $r_K\leftarrow 0$\;
$\{T[1..n],mdist[1..n],cdist[1..n]\} \gets ComputeInitialDistances(\mathcal{L}, c)$\;
{}
% \For{$i\leftarrow 1..n$}{ 
%     $maxAdj[i] \leftarrow 0$\;
%     $maxCenter[i] \leftarrow 0$\;
%     $rtDist[i] \leftarrow 0$\;
%     \For{$j\leftarrow 1..m_i$}{
%         \If{$j < m_i$ }{
%             $temDist\leftarrow d(l_i^j, l_i^{j+1})$\;
%             $rtDist[i] \leftarrow rtDist + temDist$\;
%             \If{$maxAdj < temDist$}{
%                  $maxAdj[i] \leftarrow temDist$\;
%             }
%         }
%         \If{$maxCenter_i < d_E(l_i^j, c_i)$ }{
%             $maxCenter[i] \leftarrow d_E(l_i^j, c_i)$\;
%         }
%     }
% }
$Enqueue(Q, \{root, d_E(c_K, root)\})$\;
\While{$Q\ne \phi$  and $Contains(c_K,r_K, S_1, S_2, S_3) = false$}{
	$\{p , d_E(c_K, p)\}   \gets Dequeue(Q)$\;
	$r_K \gets d_E(c_K, p)$\;
	\If{$p$ is not a POI}{
		\ForEach{$node : p.children$}{                    
		       $Enqueue(Q,\{node, d_E(c_K, node)\})$\;
		}
	}
	\ElseIf{$Prune(p, S_1, S_2, S_3) = false$}{		
		$TO_{new} \gets 0$, $L^d_{new} \gets \phi$\;
		\For{$i \gets 1..n$}{
			$\{TO[i], l^d_i\} \gets ComputeTO(p, L_i)$\;
			$TO_{new} \gets TO_{new} +TO[i]$, $L^d_{new} \gets L^d_{new} \cup \{l^d_i$\}\;
		}
		\If{$TO_{new} < TO_{opt}$}{
			 $TO_{opt} \gets TO_{new}$, $L^d \gets L^d_{new}$\; 
			 $R \gets \{p, L^d\}$\;			
			%$\{ S_1, S_2, S_3\} \gets UpdateSearchArea(\mathcal{L}, S_1, S_2, S_3, p, L^d)$\;	
                  % $\{ S_1, S_2, S_3\} \gets UpdateSearchArea(S_1,S_2,S_3,T[1..n],mdist[1..n],cdist[1..n],TO[1..n],TO_{opt})$\;
                \For{$i \gets 1..n$}{
                    $S_1[i].radius \gets \frac{TO_{opt}}{2n} + \frac{mdist[i]}{2} + cdist[i]$\;
                    $S_2[i].radius \gets \frac{TO[i]}{2} + \frac{mdist[i]}{2} + cdist[i]$\;
                    $S_3[i].radius \gets TO_{opt} + T[i]$\;
                }
                 
		}
	}
}
\Return $R$\;
\end{algorithmic}


==> sections/algos/update_search_area.tex <==
% \KwIn{$S_1, S_2, S_3$: current search areas, $TO_{opt}$: current optimal total trip overhead distance, $TO[1..n]$: current trip overhead distance for each user, $T[1..n]$: trip distance for each user without visiting any POI, $mdist[1..n]$: maximum distance between two adjacent trip locations for each user, and $cdist[1..n]$: maximum euclidean distance between a trip location and the trip centroid for each user}
% \KwOut{Return latest refined search area $S_1, S_2, S_3$}
\KwIn{$\{S_1,S_2,S_3,T[1..n],mdist[1..n],cdist[1..n],TO[1..n],TO_{opt}\}$}
\KwOut{$\{S_1, S_2, S_3\}$}
    \For{$i \gets 1..n$}{
        $S_1[i].radius \gets \frac{TO_{opt}}{2n} + \frac{mdist[i]}{2} + cdist[i]$\;
        $S_2[i].radius \gets \frac{TO[i]}{2} + \frac{mdist[i]}{2} + cdist[i]$\;
        $S_3[i].radius \gets TO_{opt} + T[i]$\;
    }
\Return \{$S_1, S_2, S_3$\}\;

==> sections/theorem/theorem_1.tex <==
\subsubsection{Pruning Technique 1 (PT1)} \label{pruning_1}
The search area can be refined as the \textbf{union} of $n$ circular regions $A_1, A_2, \dots, A_n$, where each $A_i$ is a circle having center at $c_i$ and radius as $r_i$ where the value of $r_i$ is defined as $\frac{TO(p)}{2n} + \frac{\max_{1 \leq j  \leq m_i}  d(l_i^j, l_i^{j+1})}{2} +  \max_{1 \leq j  \leq m_i} d(c_i, l_i^j)$. Theorem \ref{theorem_1} and its accompanying proof substantiates this assertion.

\begin{theorem}\label{theorem_1}
Let POI $p$ be the current optimal meetup point having the current minimum total trip overhead distance $TO(p)$. The combined region of $n$ circles $A_1 \cup A_2\cup \dots \cup A_n$ can be used as the refined search space, where each $A_i$ is a circle with center at $c_i$ and radius $r_i$ equal to $\frac{TO(p)}{2n} + \frac{\max_{1 \leq j  \leq m_i}  d(l_i^j, l_i^{j+1})}{2} +  \max_{1 \leq j  \leq m_i} d(c_i, l_i^j)$.
\end{theorem}
The proof of Theorem~\ref{theorem_1} can be found in [Author(s), Year].\\
% In the 5.3 from Hashem et al.~\cite{hashem2015efficient} shows that distance between a POI

==> sections/theorem/theorem_2.tex <==
\subsubsection{Pruning Technique 2 (PT2)} \label{pruning_2}
%Theorem~\ref{theorem_1} shows the search area is the \textbf{union} of $n$ circular regions $A_1, A_2, \dots, A_n$, where the radius of each circle is determined based on the cindividual minimum trip overhead distances.
The search area can be refined as the \textbf{union} of $n$ circular regions $A_1^2, A_2^2, \dots, A_n$, where each $A_i$ is a circle having center at $c_i$ and radius $r_i$ where the value of $r_i$ is determined as $\frac{TO_i(p)}{2} + \frac{\max_{1 \leq j  \leq m_i} d(l_i^j, l_i^{j+1})}{2} +  \max_{1 \leq j  \leq m_i} d(c_i, l_i^j)$. Theorem \ref{theorem_2} and its accompanying proof substantiates this assertion.

\begin{theorem}\label{theorem_2}
Let POI $p$ be the current optimal meetup point having the minimum total trip overhead distance $TO(p)$ and individual minimum trip overhead distances $TO_i(p)$ for every user $u_i$. The combined region of $n$ circles $A_1 \cup A_2\cup \dots \cup A_n$ can be used as the refined search space, where each $A_i$ is a circle with center at $c_i$  radius $r_i$ equal to $\frac{TO_i(p)}{2} + \frac{\max_{1 \leq j  \leq m_i} d(l_i^j, l_i^{j+1})}{2} +  \max_{1 \leq j  \leq m_i} d(c_i, l_i^j)$.
\end{theorem}

The proof of Theorem~\ref{theorem_2} can be found in [Author(s), Year].\\
% In the 5.3 from Hashem et al.~\cite{hashem2015efficient} shows that distance between a POI

==> sections/theorem/theorem_3.tex <==
% \begin{lemma}\label{lemma_1}
% Given that $c_i$ is the geometric centroid of user $u_i$’s trip locations $L_i=\{l_i^1, l_i^2, \dots, l_i^{m_i}\}$, the following inequality holds for any POI $p$: $d_E(c_i, p) \leq \frac{1}{m_i}\sum_{1 \leq j \leq m_i} d_E(l_i^j, p)$, where $d_E$ denotes the Euclidean distance.
% \end{lemma}
% Interested readers are requested to see the proof c of Hashem et al.~\cite{hashem2015efficient}.%,  ~\cite{hashem2013group}.%
\subsubsection{Pruning Technique 3 (PT3)} \label{pruning_3}
The search area can be refined as the \textbf{intersection} of $n$ circular regions $A_1, A_2, \dots, A_n$, where each $A_i$ is a circle having center at $c_i$ and radius $r_i$. The value of $r_i$ is defined as $r_i=TO(p)+T_i$, where $TO(p)$ is the  total trip overhead distance with respect to the current optimal meetup point $p$ and $T_i$ is the trip distance of user $u_i$ without visiting any POI. Theorem \ref{theorem_3} and its accompanying proof substantiates this assertion.

\begin{theorem}\label{theorem_3}
Let POI $p$ be the current optimal meetup point having the minimum total trip overhead distance $TO(p)$. The intersection region of $n$ circles $A_1 \cap A_2\cap \dots \cap A_n$ can be used as the refined search area where each $A_i$ is a circle with center at $c_i$ and radius $r_i$ equal to $TO(p)+T_i$.
\end{theorem}
The proof of Theorem~\ref{theorem_3} can be found in [Author(s), Year].\\
% In the 5.3 from Hashem et al.~\cite{hashem2015efficient} shows that distance between a POI
